Motion Prediction using Trajectory Sets and Self-Driving Domain Knowledge

Predicting the future motion of vehicles has been studied using various techniques, including stochastic policies, generative models, and regression. Recent work has shown that classification over a trajectory set, which approximates possible motions, achieves state-of-the-art performance and avoids issues like mode collapse. However, map information and the physical relationships between nearby trajectories is not fully exploited in this formulation. We build on classification-based approaches to motion prediction by adding an auxiliary loss that penalizes off-road predictions. This auxiliary loss can easily be pretrained using only map information (e.g., off-road area), which significantly improves performance on small datasets. We also investigate weighted cross-entropy losses to capture spatial-temporal relationships among trajectories. Our final contribution is a detailed comparison of classification and ordinal regression on two public self-driving datasets.

==> sections/broader_impact.tex <==
\section{Broader Impacts}
%In order to provide a balanced perspective, authors are required to include a statement of the potential broader impact of their work, including its ethical aspects and future societal consequences. 
%Authors should take care to discuss both positive and negative outcomes.

We study the problem of predicting the future motion of vehicles.
Our main contributions are to encode domain knowledge through a) the use of weighted cross-entropy losses to better capture spatial-temporal relationships, and b) adding an auxiliary loss that penalizes off-road predictions.

Our work is a key component of the broader goal to develop safe and reliable self-driving cars.
Self-driving cars hold the promise to dramatically reduce the number of fatalities and injuries due to car accidents.
Autonomous vehicles can also help improve the lives of commuters by allowing passengers to more productively use their time.
Another benefit of self-driving cars is to improve overall transportation efficiency, resulting in less pollution.
These tremendous societal benefits have led numerous companies to pursue self-driving car development.

There are potential downsides to self-driving cars as well.
Widespread adoption may displace many professional drivers.
Additionally, even if the vehicles are much safer than a human driver, accidents that result in injuries or fatalities are still possible.

Our work also has broad potential impacts for robotic systems operating in dynamic and uncertain environments - not just self-driving cars.
Examples include robots that assist humans in the home, at work, and during disaster response.
Our methods could potentially be adapted to these environments to help predict the actions of others, leading to safer and more responsive systems.
Of note, our use of domain knowledge can lead to improved interpretability.
Additionally, it can improve generalization, making it less likely that these types of models will fail in unexpected scenarios.

